OverNet: Lightweight Multi-Scale Super-Resolution with Overscaling Network

Super-resolution (SR) has achieved great success due to the development of deep convolutional neural networks (CNNs). However, as the depth and width of the networks increase, CNN-based SR methods have been faced with the challenge of computational complexity in practice. Moreover, most of them train a dedicated model for each target resolution, losing generality and increasing memory requirements. To address these limitations we introduce OverNet, a deep but lightweight convolutional network to solve SISR at arbitrary scale factors with a single model. We make the following contributions: first, we introduce a lightweight recursive feature extractor that enforces efficient reuse of information through a novel recursive structure of skip and dense connections. Second, to maximize the performance of the feature extractor we propose a reconstruction module that generates accurate high-resolution images from overscaled feature maps and can be independently used to improve existing architectures. Third, we introduce a multi-scale loss function to achieve generalization across scales. Through extensive experiments, we demonstrate that our network outperforms previous state-of-the-art results in standard benchmarks while using fewer parameters than previous approaches.

==> Tabels/Generalization.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[!t]
\caption{\small Average PSNR of state-of-the-art method CARN using OSM instead of its typical upsampling module. Best results are \textbf{highlighted}, second best are \underline{underlined}.}
\centering
\footnotesize
%\begin{adjustbox}{width=1\textwidth}
\setlength\arrayrulewidth{0.5pt}
\begin{tabular*}{\textwidth}{l@{\extracolsep{\fill}}cccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{CARN\cite{ahn2018fast}}} & \multicolumn{3}{c}{\textbf{CARN with OSM}} & \multicolumn{3}{c}{\textbf{OverNet without OSM}} & \multicolumn{3}{c}{\textbf{OverNet}} \\ 
\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} \cmidrule(l){11-13}
 & \multicolumn{1}{c}{x2} & \multicolumn{1}{c}{x3} & \multicolumn{1}{c}{x4} & \multicolumn{1}{c}{x2} & \multicolumn{1}{c}{x3} & \multicolumn{1}{c}{x4} & \multicolumn{1}{c}{x2} & \multicolumn{1}{c}{x3} & \multicolumn{1}{c}{x4} & \multicolumn{1}{c}{x2} & \multicolumn{1}{c}{x3} & \multicolumn{1}{c}{x4} \\ 
 \midrule
Set5 & 37.76 & 34.29 & 32.09 & 37.90 & 34.35 & 32.15 & \underline{38.02} & \underline{34.43} & \underline{32.23} & \textbf{38.11} &\textbf{34.49} & \textbf{32.32} \\ 
B100 & 32.09 & 29.06 & 27.58 & 32.15 & 29.10 & 27.60 & \underline{32.20} & \underline{29.12} & \underline{27.61} & \textbf{32.23} &\textbf{29.17} & \textbf{27.67} \\ 
\multicolumn{1}{l}{Urban100} & 31.92 & 28.06 & 26.07 & 32.01 & 28.12 & 26.13 & \underline{32.30} & \underline{28.27} & \underline{26.22} & \textbf{32.44} &\textbf{28.37} & \textbf{26.31} \\
\bottomrule
\end{tabular*}%
%\end{adjustbox}

\label{tab:CARN}
\end{table*}

==> Tabels/Results.tex <==
\begin{table*}[htb!]

\caption{\small Average PSNR/SSIM values for scale factors $\times$2, $\times$3 and $\times$4 with \textbf{BI} degradation. The number of parameters and multi-adds of each method are indicated  under their name. The best performance is shown \textbf{highlighted} and the second best \underline{underlined}. }
\begin{adjustbox}{width=1\textwidth}
% \scriptsize
\setlength\arrayrulewidth{1.3pt}
%  \footnotesize
\begin{tabular}{c@{~~}c@{~}c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~~}c@{~~~}c@{~~}c@{~~~}c@{~~~}c@{~~~}c}
\toprule
{\textbf{Dataset}} &  {\begin{tabular}[c]{@{}c@{}}\textbf{Scale}\\ \end{tabular}}
 & {\begin{tabular}[c]{@{}c@{}}\textbf{VDSR\cite{kim2016accurate}}\\ \textbf{0.7M / 0.6T}\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{DRCN\cite{kim2016deeply}}\\ \textbf{1.7M / 18T}\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{LapSRN\cite{lai2017deep}}\\ \textbf{0.8M / 30G}\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{DRNN\cite{tai2017image}}\\ \textbf{0.3M / 6.8T}\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{MemNet\cite{tai2017memnet}}\\\textbf{0.7M / 2.6T}\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}\textbf{SRFBN\_S\cite{li2019feedback}}\\ \textbf{0.3M / 50G}\end{tabular}} &
{\begin{tabular}[c]{@{}c@{}}\textbf{OISR\_LF\_s\cite{he2019ode}}\\ \textbf{1.4M / 0.26T}\end{tabular}} &
 {\begin{tabular}[c]{@{}c@{}}\textbf{CARN\cite{ahn2018fast}}\\ \textbf{1.6M / 0.2T}\end{tabular}} &  
{\begin{tabular}[c]{@{}c@{}}\textbf{MSRN\cite{li2018multi}}\\ \textbf{6M / 1T}\end{tabular}}& {\begin{tabular}[c]{@{}c@{}}\textbf{OverNet}\\ \textbf{0.9M / 0.2T}\end{tabular}} \\ 
\midrule
{Set5} & {\begin{tabular}[c]{@{}l@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}37.53/0.9587\\ 33.66/0.9213\\ 31.35/0.8838\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}37.63/0.9588\\ 33.82/0.9226\\ 31.53/0.8838\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}37.52/0.9591\\ 33.82/0.9227\\ 31.54/0.886\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}37.74/0.9591\\ 34.03/0.9244\\ 31.68/0.8888\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}33.78/0.9597\\ 34.09/0.9245\\ 31.74/0.8893\end{tabular}} & 
{\begin{tabular}[c]{@{}c@{}}37.78/0.9156\\ 34.20/0.9255\\ 31.98/0.8923\end{tabular}} &{\begin{tabular}[c]{@{}c@{}}38.02/0.9605\\ 34.39/0.9272\\ 32.14/0.8947\end{tabular}}  &
{\begin{tabular}[c]{@{}c@{}}37.76/0.9590\\ 34.29/0.9255\\ 32.13/0.8932\end{tabular}} &
{\begin{tabular}[c]{@{}c@{}}\underline{38.08}/\underline{0.9605}\\ \underline{34.38/0.9262} \\ \underline{32.07/0.8903}\end{tabular}}&{\begin{tabular}[c]{@{}c@{}}\textbf{38.11}/\textbf{0.9602}\\ \textbf{34.49}/\textbf{0.9536}\\ \textbf{32.32}//\textbf{0.9023}\end{tabular}}  \\ 
\midrule
{Set14} & {\begin{tabular}[c]{@{}l@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}33.05/0.9127\\ 29.78/0.8318\\ 28.02/0.7678\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}33.06/0.9121\\ 29.77/0.8314\\ 28.03/0.7673\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}32.99/0.9124\\ 29.79/0.8320\\ 28.09/0.7994\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}33.23/0.9136\\ 29.96/0.8349\\ 28.21/0.7720\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}33.28/0.9142\\ 30.00/0.8350\\ 28.26/0.7723\end{tabular}} & 
{\begin{tabular}[c]{@{}c@{}}33.35/0.9156\\ 30.10/0.8372\\ 28.45/0.7779\end{tabular}} &{\begin{tabular}[c]{@{}c@{}}33.62/0.9178\\ 30.35/0.8426\\ 28.63/0.7819\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}33.52/0.9166\\ 30.29/0.8407\\ 28.60/0.7806\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{33.74}/\textbf{0.9013}\\ \underline{30.34/0.8437}\\ \underline{28.60/0.7836}\end{tabular}}&
{\begin{tabular}[c]{@{}c@{}}\underline{33.71/0.9180}\\ \textbf{33.45}/\textbf{0.8058}\\ \textbf{28.67}/\textbf{0.8734}\end{tabular}}\\
 
\midrule
{B100} & {\begin{tabular}[c]{@{}l@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}31.90/0.8960\\ 28.83/0.7976\\ 27.29/0.7252\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}31.85/0.8942\\ 28.80/0.7963\\ 27.24/0.7233\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}31.80/0.8949\\ 28.82/0.7973\\ 27.32/0.7264\end{tabular}} & {\begin{tabular}[c]{@{}l@{}}32.05/0.8973\\ 28.95/0.8004\\ 37.38/0.7284\end{tabular}} & 
{\begin{tabular}[c]{@{}c@{}} 32.00/0.8970\\ 28.96/0.8010\\ 27.44/0.7313\end{tabular}} &{\begin{tabular}[c]{@{}l@{}}32.20/0.9000\\ 29.11/0.8085\\ 27.60/0.7369\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}32.08/0.8984\\ 28.97/0.8025\\ 27.44/0.7325\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}32.09/0.8978\\ 29.06/0.8034\\ 27.58/0.7349\end{tabular}} &

{\begin{tabular}[c]{@{}c@{}}\underline{32.22/0.8993}\\ \textbf{29.13}/\textbf{0.7936}\\ \textbf{27.65}/\textbf{0.7589}\end{tabular}} &

{\begin{tabular}[c]{@{}c@{}}\textbf{32.23}/\textbf{0.9002} \\ \underline{29.08/0.8041}\\ \underline{27.52/0.7273}\end{tabular}}   \\
\midrule
{Urban100} & {\begin{tabular}[c]{@{}l@{}}$\times$2\\ $\times$3\\ $\times$4\end{tabular}} &  {\begin{tabular}[c]{@{}c@{}}30.77/0.9141\\ 27.14/0.8279\\ 25.18/0.7525\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}30.76/0.9133\\ 27.15/0.8277\\ 25.14/0.7511\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}30.41/0.9101\\ 27.07/0.8271\\ 25.21/0.7553\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}31.23/0.9188\\ 27.53/0.8377\\ 25.44/0.7638\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}31.31/0.9195\\ 27.56/0.8376\\ 25.50/0.7630\end{tabular}}  &
{\begin{tabular}[c]{@{}c@{}}31.41/0.9207\\ 26.41/0.8064\\ 24.60/0.7258\end{tabular}} &{\begin{tabular}[c]{@{}c@{}}32.21/0.9290\\ 28.24/0.8544\\ 26.17/0.7888\end{tabular}}  &  {\begin{tabular}[c]{@{}c@{}}31.92/0.9256\\ 28.06/0.8493\\ 26.07/0.7837\end{tabular}}
&{\begin{tabular}[c]{@{}c@{}}\underline{32.22/0.9326}\\ \underline{28.08/0.8554}\\ \underline{26.04/0.7896}\end{tabular}}&   
{\begin{tabular}[c]{@{}c@{}}\textbf{32.44}/\textbf{0.8679}\\ \textbf{28.37}/\textbf{0.8754}\\ \textbf{26.25}/\textbf{0.8112}\end{tabular}}
\\ 
\bottomrule

\end{tabular}
\end{adjustbox}

\label{tab:results}
\end{table*}

==> draft.tex <==


 The extracted features by a deep network contain different types of information across channels. If we are able to increase the network's sensitivity to information-rich channels and make it focus on them, the representational power of the network would be enhanced and the performance improved. 
